Understanding Incremental Learning of Gradient Descent: A Fine-grained Analysis of Matrix Sensing

It is believed that Gradient Descent (GD) induces an implicit bias towards good generalization in training machine learning models. This paper provides a fine-grained analysis of the dynamics of GD for the matrix sensing problem, whose goal is to recover a low-rank ground-truth matrix from near-isotropic linear measurements. It is shown that GD with small initialization behaves similarly to the greedy low-rank learning heuristics (Li et al., 2020) and follows an incremental learning procedure (Gissin et al., 2019): GD sequentially learns solutions with increasing ranks until it recovers the ground truth matrix. Compared to existing works which only analyze the first learning phase for rank-1 solutions, our result provides characterizations for the whole learning process. Moreover, besides the over-parameterized regime that many prior works focused on, our analysis of the incremental learning procedure also applies to the under-parameterized regime. Finally, we conduct numerical experiments to confirm our theoretical findings.

==> Sections/experiments.tex <==



In this section, we perform numerical experiments to empirically verify our theoretical findings.
%\simon{Need to make the legends, labels, captions bigger.}



\begin{comment}
\begin{figure*}[t]
    %\vspace{-0.25in}
    \centering
    \begin{subfigure}[c]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/low_rank_exact0.png}
        \caption[]%
        {{\small $\alpha=1$, $1000$ measurements.}}    
        \label{low_rank_exact0}
    \end{subfigure}
    \qquad
    \begin{subfigure}[c]{0.3\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_exact1.png}
        \caption[]%
        {{\small $\alpha=0.1$, $1000$ measurements.}}    
        \label{low_rank_exact1}
    \end{subfigure}
    \vskip\baselineskip\vspace{-0.15in}
    \begin{subfigure}[c]{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_exact2.png}
        \caption[]%
        {{\small $\alpha=0.01$, $1000$ measurements.}}    
        \label{low_rank_exact2}
    \end{subfigure}
    \qquad
    \begin{subfigure}[c]{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_exact3.png}
        \caption[]%
        {{\small $\alpha=0.001$, $1000$ measurements.}}    
        \label{low_rank_exact3}
    \end{subfigure}
    \caption[]%
    {The evolution of the loss and relative error against best solution of different ranks in the exact-parameterized case $r=5$.}
    \label{low_rank_exact}
\end{figure*}
\end{comment}



\textbf{Experimental setup.} We consider the matrix
sensing problem \Cref{matrix-sensing} with $d=50$, $r_*=5$,
$\alpha\in\left\{1,0.1,0.01,0.001\right\}$, $m\in\left\{1000,2000,5000\right\}$.
We will consider different choices for $\hr$ in the experiments. The ground truth
$\mZ^* = \mX\mX^{\top}$ is generated such that the entries of $\mX$ are i.i.d.
standard Gaussian variables.
We use the same
ground truth throughout our experiments.
% to compare different choices of parameters. 

For
$i=1,2,\cdots,m$, all entries of the measurement $\mA_i\in\R^{d\times d}$ are chosen i.i.d. from the standard Gaussian $\mathcal{N}(0,1)$.  When
$m \gtrsim d r_*\delta^{-2}$, this set of measurements satisfies the RIP with
high probability~\citep[Theorem 4.2]{recht2010guaranteed}.


We solve the problem \Cref{matrix-sensing} via running GD for $T=10^4$
iterations starting with small initialization with scale $\alpha$. Specifically,
we choose $\mU_0 = \alpha\bar{\mU}$ where the entries of $\bar{\mU}\in\R^{d\times \hr}$ are
drawn i.i.d.~from $\mathcal{N}(0,1)$. We consider both the
over-parameterized and the exact/under-parameterized regime. The learning rate
of GD is set to be $\mu=0.005$.



\subsection{Implicit low-rank bias}

In this subsection, we consider the over-parameterized setting with $r=50$. %As defined \Cref{sec-prelim}, let $\mZ^* = \sum_{i=1}^{r^*}\sigma_i^2\vv_i\vv_i^{\top}$ and $\mX_s\mX_s^{\top} = \sum_{i=1}^{s}\sigma_i^2\vv_i\vv_i^{\top}$. 
For each iteration $t \in [T]$ and rank $s \in [r_*]$, we define the relative error $\mathcal{E}_s(t) = \frac{\left\|\mU_t\mU_t^{\top}-\mX_s\mX_s^{\top}\right\|_F^2}{\left\|\mX_s\mX_s^{\top}\right\|_F^2}$ to measure the proximity of the GD iterates to $\mX_s$. We plot the relative error in \Cref{low_rank} for different choices of $\alpha$ and $m$ (which affects the measurement error $\delta$).


\textbf{Small initialization.} The implicit low-rank bias of GD is evident when
the initialization scale $\alpha$ is small. Indeed, one can observe that GD
first visits a small neighborhood of $\mX_1$, spends a long period of time near
it, and then moves towards $\mX_2$. It then proceeds to learn
$\mX_3,\mX_4,\cdots$ in a similar way, until it finally fits the ground truth.
This is in align with \Cref{main_result}. By
contrast, for large initialization we do not have this implicit bias.

\textbf{The effect of measurement error.} For fixed $\alpha$, one can observe
the relative error becomes smaller when the number of measurements increases.
This is in align with \Cref{main-lemma} in which the bound
depends on $\delta$. In particular, for the case $s=r_*$, in the end the distance to the set
of global minima goes to zero as $\alpha \to 0$.
%\kaifeng{it is hard to see whether it is poly or not. Maybe just say something qualitatively?}


\subsection{Matrix sensing with exact parameterization}

Now we study the behavior of GD in the exact parameterization regime ($r=r_*$).
We fix $m=1000$, $r=r_*=5$ and run GD for $T=500$ iterations. We plot the
relative error in \Cref{low_rank_exact}.
As predicted by \Cref{main_result}, we can observe that when $\alpha$ is small, GD exhibits an implicit low-rank bias and takes a longer time to converge.
The latter is because GD would get into a $\mathrm{poly}(\alpha)$-small neighborhood of the
saddle point $\mZ_s$ and take a long time to escape the saddle. As guaranteed by \Cref{main-thm-cor}, we also observe the final convergence to global minimizers for sufficiently small $\alpha$.
%\kaifeng{I cannot understand the last sentence. What is "Also" for?}



==> Sections/landscape.tex <==

%Our analysis in \Cref{sec-main-result} provides technical tools for proving the following corollary.

%With the help of the landscape results in \Cref{sec-landscape}, we obtain the following corollary which states that when $r \leq r_{*}$, GD with a small initialization can actually find global minima of \Cref{under-param-sensing}. 

\begin{figure*}
    \centering
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/low_rank_bias0.png}
        \caption[]%
        {{\small $\alpha=1$, $1000$ measurements.}}    
        \label{low_rank0}
    \end{subfigure}
    \qquad
    \begin{subfigure}{0.3\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_bias1.png}
        \caption[]%
        {{\small $\alpha=0.1$, $1000$ measurements.}}    
        \label{low_rank1}
    \end{subfigure}
    \qquad
    \begin{subfigure}{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_bias2.png}
        \caption[]%
        {{\small $\alpha=0.01$, $1000$ measurements.}}    
        \label{low_rank2}
    \end{subfigure}
    \vskip\baselineskip\vspace{-0.1in}
    \begin{subfigure}{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_bias3.png}
        \caption[]%
        {{\small $\alpha=0.001$, $1000$ measurements.}}    
        \label{low_rank3}
    \end{subfigure}
    \qquad
    \begin{subfigure}{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_bias4.png}
        \caption[]%
        {{\small $\alpha=0.001$, $2000$ measurements.}}    
        \label{low_rank4}
    \end{subfigure}
    \qquad
    \begin{subfigure}{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_bias5.png}
        \caption[]%
        {{\small $\alpha=0.001$, $5000$ measurements.}}    
        \label{low_rank5}
    \end{subfigure}
    \caption[]%
    {The evolution of relative error against the best solution of different ranks over time.} 
    \label{low_rank}
\end{figure*}

In this section, we analyze the properties of
the landscape of the matrix sensing loss \Cref{matrix-sensing}, which plays a crucial role in proving results in \Cref{sec-main-result}. While the
landscape of over-parameterized matrix sensing (i.e. $\hr\geq r^*$) is
well-studied \citep{tu2016low,ge2017no}, few results are known for the
under-parameterized case. %A strict saddle property of matrix factorization is
%established in \citet{zhu2021global}, but this does not necessarily imply that
%GD converges to global minima \citep{du2017gradient} with a fast rate.
Our results provide useful tools for analyzing the convergence of gradient-based algorithms for solving problems like low-rank matrix approximation and  might have independent interests.
% since low-rank matrix approximation itself is an
% active research area
% \citep{lee2013local,kishore2017literature,tropp2019streaming} and is also of
% practical importance \citep{chen2017denoising,lu2020low}.


To prove convergence results like \Cref{main-thm-cor},  we first study the landscape of $f_s$ defined in \Cref{under-param-sensing} near the set of global minimizers. One major difficulty here is that $f_s$ is not locally strongly-convex, because if $\mU\in\R^{d\times s}$ is a global minimizer of $f_s$, then $\mU\mR$ is also a global minimizer, for any orthogonal matrix $\mR\in\R^{s\times s}$ . Nonetheless, we can establish a Polyak-\L{}ojasiewicz (PL) like condition,~\Cref{landscape-main-thm}, which is the main result of this section.
% with respect to the procrustes distance defined below. 






When $\delta=0$, $f_s$ reduces to the matrix factorization loss $F_s:\R^{d\times s}\to \R, F_s(\mU) = \frac{1}{4d^2}\left\|\mU\mU^{\top}-\mZ^*\right\|_F^2$.
%The following corollary immediately follows from \Cref{landscape-main-thm}.

\begin{corollary}[Landscape of under-parameterized matrix factorization] 
\label{matrix-fact-landscape}
The set of global minimizers of $F_s$ is $\left\{\mX_s\mR: \mR\in\R^{s\times s} \textit{ is orthogonal}\right\}$. Moreover, under \Cref{asmp:rip}, given $\mU\in\R^{d\times s}$ and let $\mR$ be an orthogonal matrix such that $\left\|\mU-\mX_s \mR\right\|_F = \mathrm{dist}(\mU,\mX_s)$. If $\mathrm{dist}(\mU,\mX_s) \leq 10^{-2}\kappa^{-1}\|\mX\|$, then $\left\langle \nabla F(\mU), \mU - \mX_s \mR \right\rangle \geq 0.1\tau\mathrm{dist}^2(\mU,\mX_s)$.
\end{corollary}




\begin{comment}
\begin{proof-sketch}
    The definition of $\mU_s^*$ implies that $\mU^{\top}\mU_s^*$ is positive semi-definite. Let $\mH=\mU-\mU_s^*$, then we have
    \begin{equation}
        \notag
        \begin{aligned}
        \nabla f_s(\mU) 
        &= \left(\A^*\A\right)\left[ (\mH + \mU_s^*)(\mH + \mU_s^*)^{\top} - \mX \mX^{\top}\right] (\mH + \mU_s^*) \\
        &= \left[\left(\A^*\A\right)\left( \mH \mH^{\top} + \mU_s^* \mH^{\top} + \mH \left(\mU_s^*\right)^{\top}\right)\right] (\mH+\mU_s^*) - \A^*\A \left( \mX \mX^{\top} - \mU_s^*\left(\mU_s^*\right)^{\top}\right) \mH
        \end{aligned}
    \end{equation}
    where we use the first-order optimality condition $\nabla f_s(\mU_s^*) = \A^*\A \left( \mX \mX^{\top} - \mU_s^*\left(\mU_s^*\right)^{\top}\right) \mU_s^* = 0$. Using the RIP property, it follows that
    \begin{equation}
        \notag
        \begin{aligned}
        &\quad \left\langle \nabla f_s(\mU), \mU - \mU_s^*\right\rangle \\
        &\geq \left\langle \left( \mH \mH^{\top} + \mU_s^*\mH^{\top} + \mH \left(\mU_s^*\right)^{\top}\right) (\mH+\mU_s^*) -  \left( \mX \mX^{\top} - \mU_s^*\left(\mU_s^*\right)^{\top}\right) \mH, \mH \right\rangle -\O\left(\delta\|\mX\|^2\|\mH\|_{F}^2\right) \\
        &\geq \mathrm{tr}\left(\mH(\mH+\mU_s^*)^{\top} (\mH+\mU_s^*)\mH^{\top}+\mH^{\top} \mU_s^* \mH^{\top} \mH + \left( \left(\mU_s^*\right)^{\top} \mH\right)^2 \right.\\
        &\quad \left.- \mH^{\top} \left( \mX \mX^{\top} - \mU_s^*\left(\mU_s^*\right)^{\top}\right) \mH\right) -\O\left(\delta\|\mX\|^2\|\mH\|_F^2\right) \\
        &\geq \left[\underbrace{\sigma_{\min}\left(\left(\mU_s^*\right)^{\top} \mU_s^*\right)}_{\approx \sigma_s^2} - \underbrace{\left\|\mX \mX^{\top} -\mU_s^*\left(\mU_s^*\right)^{\top}\right\|}_{\approx \sigma_{s+1}^2}-\O\left(\delta\|\mX\|^2\right)-3\|\mU_s^*\|\|\mH\| - \|\mH\|^2\right] \|\mH\|_F^2 \\
        &\gtrsim 0.1\tau_s\|\mH\|_F^2
        \end{aligned}
    \end{equation}
    under given conditions on $\mH$ and $\delta$, which yields the desired conclusion.
\end{proof-sketch}

We conclude this section with the following corollary which states that the global minimizer of the under-parameterized loss \Cref{under-param-sensing} is unique.

\begin{corollary}
    Under the conditions in \Cref{landscape-main-thm}, the global minimizer of $f_s$ is unique up to rotation i.e. for any two minimizer $\mU_1$ and $\mU_2$, there must exists an orthogonal matrix $\mR$ such that $\mU_1 = \mU_2 \mR$.
\end{corollary}
\end{comment}

==> Sections/main-result-revised.tex <==
In this section, we present our main theorems and their proof sketches,
following the theoretical setup in \Cref{sec-prelim}. Full proofs can be found
in \Cref{appsec:thm-fit,appsec-aux,appsec-landscape,appsec-main-proof}.

\begin{restatable}[]{theorem}{mainThm} \label{main_result}
Under \Cref{asmp:rip,asmp-full-rank,asmp:step-size},
consider GD~\Cref{GD}
with initialization $\mU_{\alpha, 0} = \alpha \bmU$
for solving the matrix sensing problem~\Cref{matrix-sensing}. 
There exist universal constants $c, M$, constant $C = C(\mX,\bar{\mU})$ %, an exponent $\gamma \ge \frac{1}{10 \kappa}$ 
and a sequence of time points $T_{\alpha}^1<T_{\alpha}^2<\cdots<T_{\alpha}^{\hr\wedge r_*}$ %(depending on $\alpha$)
such that
for all $1 \le s \le \hr \land r_*$, 
the following holds when $\alpha$ is sufficiently small:
\begin{equation}
    \normF{\mU_{\alpha, T_{\alpha}^{s}} \mU_{\alpha, T_{\alpha}^{s}}^\top - \mZ_s^*} \le C \alpha^\frac{1}{M\kappa^2},
\end{equation}
where we recall that $\mZ_s^*$ is the best rank-$s$ solution defined in \Cref{def:best-rank}.
Moreover, GD follows an incremental learning procedure: we have $\lim_{\alpha\to 0}\max_{1\leq t\leq T_{\alpha}^s}\sigma_{s+1}(\mU_{\alpha,t})=0$ for all $1\leq s\leq \hr\wedge r_*$, where $\sigma_{i}(\mA)$ denotes the $i$-th largest singular value of a matrix $\mA$.%\zhiyuan{@jikai, clarify what $\lesssim$ means}


%with initialization $\mU_{\alpha, t} = \alpha \mU$,
%there exist positive integers $T_{\alpha}^1<T_{\alpha}^2<\cdots<T_{\alpha}^{r\wedge r_*}$ such that $\lim_{\alpha\to 0}\max_{1\leq i\leq r\wedge r_*}\left\|\mU_{\alpha,T_{\alpha}^i}\mU_{\alpha,T_{\alpha}^i}^\top-\mZ_i\right\| = 0$
\end{restatable}
%\zhiyuan{@jikai, (1) no need to introduce $\gamma$ here, just use $\alpha^{\frac{1}{10\kappa}}$; (2) $T_\alpha$ depending on $\alpha$ seems trivial; (3). what is $r$; (4) $c$ undefined}

It is guaranteed that $\mZ_s^*$ is unique for all $1\leq s\leq \hr\wedge r_*$
under our assumptions (see \Cref{landscape-main-global-unique}). In short,
\Cref{main_result} states that GD with small initialization discovers the best
rank-$s$ solution ($s=1,2,\cdots,\hr\wedge r_*$) sequentially. In particular,
when $s=r_*$, the best rank-$s$ solution is exactly the ground truth
$\mX\mX^\top$. Hence with over-parameterization ($\hr\geq r_*$), GD can discover
the ground truth. %\zhiyuan{why can $s=\hat{r}$, if $\hr\geq r_*$?}

At a high level, our
result characterizes the complete learning dynamics of GD and reveals an
incremental learning mechanism, \emph{i.e.}, GD starts from learning simple
solutions and then gradually increases the complexity of search space until it
finds the ground truth. %\zhiyuan{but do we have stronger assumptions?}

%From an optimization perspective, our analysis shows that GD follows a saddle-to-saddle dynamics \citep{jacot2021deep}. Theoretical studies of this dynamics are often restricted to the rank-$1$ case, since extending to higher ranks requires knowledge on how GD approaches the rank-$1$ saddle \citep{li2020towards}. We show that for matrix sensing problems, GD approaches the rank-$s$ saddle through a specific trajectory that approximately lies in the rank-$s$ solution space, which in turn allows GD to efficiently escaping it. The proof idea of \Cref{thm-main} is similar to ~\cite[Theorem 5.6]{li2020towards} which shows that GF with infinitesimal initialization behaves like a rank-$1$ GF, but it is unknown whether the rank-$1$ GF converges to the minimizer for general PSD-constrained optimization problems.

In the under-parameterized setting, we can further establish the following convergence result:

\begin{restatable}[Convergence in the under-parameterized regime]{theorem}{mainThmUnderParam}
\label{main-thm-cor}
    Suppose that $\hr\leq r^*$, then there exists a constant $\bar{\alpha}>0$
    such that when $\alpha<\bar{\alpha}$, we have $\lim_{t\to
    +\infty}\mU_{\alpha,t}\mU_{\alpha,t}^{\top}=\mZ_{\hr}^*$.
\end{restatable}

\subsection{Key lemmas}
\label{subsec:key-lemma}

In this section, we present some key lemmas for proving our main results. First, we can show that with small initialization, GD can get into a small neighborhood of $\mZ_s^*$.

\begin{restatable}[]{lemma}{mainLemma} \label{main-lemma}
%There exists $\hat{\mU}_{\alpha,t} \in \R^{d \times s}$ and $\hat{\mR}_{\alpha,t} \in \R^{s \times \hr}$ for each $\alpha > 0$ and $t \in [-T_\alpha^s,0]$ to approximate $\mU_{\alpha, t+T_{\alpha}^s}$ as $\hat{\mU}_{\alpha,t} \hat{\mR}_{\alpha,r}$ in the sense such that $\lim_{\alpha \to 0} \max_{t\in[-T_\alpha^s,0]} \normF{\hat{\mU}_{\alpha, t}\hat{\mR}_{\alpha,t} - \mU_{\alpha, t+T_{\alpha}^s}} = 0$, where $T_\alpha^s$ is defined in \Cref{thm-fit-ground-truth}. Moreover, we have $\normF{\hat{\mU}_{\alpha,0} - \mU_s^*} \lesssim \kappa^2\sqrt{r_*}\|\mX\|\delta$ for some global minimizer $\mU_s^*$ of $f_s$ and $\hat{\mR}_{\alpha,t}\hat{\mR}_{\alpha,t}^\top = \mI$.%\zhiyuan{$T_\alpha$ not defined} \zhiyuan{$f_s$ hasn't been defined}
Under \Cref{asmp:rip,asmp-full-rank}, there exists $\hat{T}_{\alpha}^s>0$ for
all $\alpha>0$ and $1\leq s\leq \hr\wedge r_*$ such that $\lim_{\alpha\to
0}\max_{1\leq t\leq \hat{T}_{\alpha}^s}\sigma_{s+1}(\mU_{\alpha,t})=0$.
Furthermore, it holds that
$\left\|\mU_{\hat{T}_{\alpha}^s}\mU_{\hat{T}_{\alpha}^s}^\top -\mZ_s^*\right\|_F
=\O\left(\kappa^3 r_*\delta\|\mX\|^2\right)$.
\end{restatable}

The full proof can be found in \Cref{appsec:thm-fit}.
Motivated by \citet{stoger2021small},
we consider the following decomposition of $\mU_t$:
\begin{equation}
    \label{ut-decompose}
    \mU_t = \mU_t\mW_t\mW_t^{\top}+\mU_t\mW_{t,\perp}\mW_{t,\perp}^{\top},
\end{equation}
where %$\mW_t \in \R^{r\times s}$ is defined by 
$\mW_t := \mW_{\mV_{\mX_s}^{\top}\mU_t} \in \R^{\hr \times s}$ is the matrix
consisting of the right singular vectors of $\mV_{\mX_s}^{\top}\mU_t$
(\Cref{def:svd}) and $\mW_{t,\perp} \in \R^{\hr \times (\hr-s)}$ is any
orthogonal complement of $\mW_t$, \emph{i.e.}, $\mW_{t}\mW_{t}^\top +
\mW_{t,\perp}\mW_{t,\perp}^\top = \mI$. The dependence of $\mW_{t},\mW_{t,\perp}$
on $s$ is omitted but will be clear from the context.

We will refer to the term $\mU_t\mW_t\mW_t^\top$ as the \textit{parallel component} and
$\mU_t\mW_{t,\perp}\mW_{t,\perp}^\top$ as the \textit{orthogonal component}. The idea is to
show that the parallel component grows quickly until it gets close to the best
rank-$s$ solution at some time $\hat{T}_{\alpha}^s$ (namely $\mU_t\mW_t\mW_t^\top\mU_t^\top \approx \mZ_s^*$ when $t = \hat{T}_{\alpha}^s$). Meanwhile, 
the orthogonal term grows exponentially slower and stays $o(1)$ before $\hat{T}_{\alpha}^s$.
See 
\Cref{sec-proof-sketch}
for a detailed proof
sketch.

\Cref{main-lemma} shows that
$\mU_t \mU_t^\top$ would enter a neighborhood of $\mZ_s^*$ with
\textit{constant} radius. However, there is still a gap between
\Cref{main-lemma} and \Cref{main_result}, since the latter states that $\mU_t
\mU_t^\top$ would actually get $o(1)$-close to $\mZ_s^*$.

To proceed, we define the \textit{under-parameterized} matrix sensing loss $f_s$
for every $1\leq s \leq r_*$:
\begin{equation}
    \label{under-param-sensing}
    f_s(\mU) = \frac{1}{4}\left\|\A(\mZ^*-\mU\mU^{\top})\right\|_2^2,\quad \mU\in\R^{d\times s}.
\end{equation}
While the function we are minimizing is $f$ (defined in \Cref{matrix-sensing}) rather than $f_s$, \Cref{main-lemma} suggests that for $t \leq \hat{T}_{\alpha}^s$, $\mU_t$ is always approximately rank-$s$, so that we use a low-rank approximation for $\mU_{\hat{T}_{\alpha}^s}$ and associate the dynamics locally with the
GD dynamics of $f_s$. We will elaborate on how this is done in \Cref{subsec:proof-outline}.


When $\mathrm{dist}(\mU_1,\mU_2) = 0$, it can be easily shown that $f_s(\mU_1) = f_s(\mU_2)$ since $f_s$ is invariant to orthogonal transformations.
Moreover, we note that the global minimizer of $f_s$ is unique up to orthogonal transformations.
%\kaifeng{remember to add a proof}
\begin{restatable}{lemma}{mainGlobalUnique}
    \label{landscape-main-global-unique}
    Under \Cref{asmp:rip}, if $\mU_s^* \in \R^{d\times s}$ is a global minimizer of $f_s$,
then the set of global minimizers
$\argmin f_s$ is equal to $\left\{\mU_s^*\mR: \mR\in\R^{s\times s}, \mR^\top \mR = \mI \right\}$.
\end{restatable}
Around the global minimizers, we show that $f_s$
satisfies the Restricted Secant Inequality (RSI) which is useful for optimization analysis.
%a Polyak-\L{}ojasiewicz (PL) type condition with respect to the procrutes distance.
\begin{restatable}[]{definition}{procrustesProjection}
    \label{def:procrutes-projection}
    For any $\mU \in \R^{d \times s}$, 
    we use $\Pi_s(\mU)$ to denote the set of {\em closest} global minimizers of
    $f_s$ to $\mU$, namely 
    $\Pi_s(\mU) = \argmin\{\|\mU - \mU^*_s\|_F: \mU^*_s \in \argmin f_s \}$.
\end{restatable}
\begin{restatable}[Restricted Secant Inequality]{lemma}{mainLandscape}
    \label{landscape-main-thm}
    Under \Cref{asmp:rip},
    if 
    a matrix $\mU\in\R^{d\times s}$ satisfies 
    $\left\|\mU- \mU_s^* \right\|_F \leq 10^{-2}\kappa^{-1}\|\mX\|$
    for some $\mU_s^* \in \Pi_s(\mU)$,
    then we have
    \begin{equation}
    \left\langle \nabla f_s(\mU), \mU -
    \mU_s^*\right\rangle \geq 0.1\kappa^{-1}\|\mX\|^2
    \| \mU - \mU_s^* \|_F^2.
    \end{equation}
\end{restatable}

%\begin{remark}
    % A function $g:\R^n\mapsto\R$ satisfies the $(\mu,r)$- local Polyak-\Lojasiewicz (PL) condition if $\left\|\nabla g(x)\right\|^2 \geq 2\mu\left( g(x)-\min_{y\in\R^n} g(y)\right)$ when $\min\left\{ \left\|x-z\right\|: g(z)=\min_{y\in\R^n} g(y)\right\} \leq r$. 
    %Recall that PL condition for a differentiable function $g:\R^n\to\R$ means there exists some constant $\mu>0$, such that $ \left\|\nabla g(x)\right\|^2 \geq 2\mu\left( g(x)-\min_{y\in\R^n} g(y)\right)$ holds for all $x$. 
    %Since $f_s$ is locally smooth around $\mU_s^*$, there exists $L_1>0$ such that $f_s(\mU)-f_s(\mU_s^*) \leq L_1\left\|\mU-\mU_s^*\right\|_F^2$. Moreover, \Cref{landscape-main-thm} implies that $\left\|\mU-\mU_s^*\right\|_F^2 \leq 10\|\mX\|^2\kappa^{-1}\left\|\nabla f_s(\mU)\right\|_F$, so we have $\left\|\nabla f_s(\mU)\right\|_F^2 \geq 0.01\|\mX\|^4\kappa^{-2} L_1^{-1}\left(f_s(\mU)-f_s(\mU_s^*)\right)$. In other words, \Cref{landscape-main-thm} implies that the matrix sensing loss \Cref{matrix-sensing} is locally PL.
%\end{remark}
\begin{remark}
    In general, 
    a function $g:\R^n\mapsto\R$ satisfies
    the RSI condition if for some $\mu > 0$, $\langle \nabla g(x), x-\pi(x)\rangle \ge \mu \|x-\pi(x)\|^2$ holds for all $x$,
    where $\pi(x)$ is a projection of $x$ onto $\argmin g$.
    This condition 
    can be used to prove linear convergence of GD~\citep{zhang2013gradient},
    but it is weaker than strong convexity and stronger than \PLfull  (PL) condition~\citep{karimi2016linear}.
    %Here \Cref{landscape-main-thm} shows that a local version of the RSI condition holds for matrix sensing under RIP.
    %$(\mu,r)$- local Polyak-\Lojasiewicz (PL) condition if $\left\|\nabla g(x)\right\|^2 \geq 2\mu\left( g(x)-\min_{y\in\R^n} g(y)\right)$ when $\min\left\{ \left\|x-z\right\|: g(z)=\min_{y\in\R^n} g(y)\right\} \leq r$. 
\end{remark}

We end this subsection with the following lemma which says that all global minimizers of the $f_s$ must be close to $\mX_s$ under the procrustes distance, which is used in the proof sketch of \Cref{main_result} in \Cref{sec-main-result}.

%\zhiyuan{condition of theorem 5.1 is unclear.}
\begin{restatable}[]{lemma}{minimaClose}
\label{lemma:minima-close}
Under \Cref{asmp:rip}, we have $\mathrm{dist}(\mU_s^*,\mX_s) \leq 40\delta\kappa\|\mX\|_F$ for any global minimizer $\mU_s^*$ of $f_s$. Moreover, $\left\|\mZ_s^*-\mX_s\mX_s^\top\right\|_F \leq 160\delta\kappa\sqrt{r_*}\|\mX\|^2$.
\end{restatable}

\begin{restatable}[]{corollary}{minimaCloseCor}
\label{cor:minima-close}
Under \Cref{asmp:rip}, we have $\sigma_{\min}(\mU_s^*) \geq \frac{1}{2} \sigma_{\min}(\mX_s) = \frac{1}{2}\sigma_s \ge \frac{1}{2} \kappa^{-\frac{1}{2}} \|\mX\|$.
\end{restatable}

The full proofs for \Cref{landscape-main-thm,lemma:minima-close,cor:minima-close} can be found in \Cref{appsec-landscape}.

%\zhiyuan{@jikai, proof of lemma 4.7, corollary 4.8 are missing}

%It can be shown that under \Cref{asmp:rip} , the global minimizer of $f_s$ is unique up to rotation, i.e., if $\hat{\mU}^*_s$ is a global minimizer of $f_s$, then any other global minimizer can be written as $\hat{\mU}^*_s \mR$ for some orthogonal matrix $\mR \in \R^{s \times s}$. The main observation is that GD follows an approximate low-rank trajectory until it gets into a small neighborhood of $\mZ_s^*$, so that we can still use our landscape results in the low-rank regime.

\subsection{Proof outline}
\label{subsec:proof-outline}

Based on the key lemmas, here we provide the outlines of the proofs for our main theorems
and defer the details to \Cref{appsec-main-proof}.
%In the following, we fix an integer $1\leq s \leq \hr\wedge r_*$ and show the existence of $T_{\alpha}^s > 0$ satisfying that $\lim_{\alpha\to 0} \normF{\mU_{\alpha,T_{\alpha}^s}\mU_{\alpha,T_{\alpha}^s}^\top-\mZ^*_s} = 0$. We then show that $T_{\alpha}^s$ is monotone increasing in $s$ for any fixed $\alpha$.
%Our key lemma states below that with small initialization, GD can get into a small neighborhood of $\mZ_s^*$. A proof sketch of \Cref{main-lemma} is detailed in \Cref{sec-proof-sketch}. 
%\zhiyuan{doesn't sound correct grammatically, an algorithm is not supposed to approximate a solution. Maybe say GD can get that close to $Z^*_s$}
%We prove this result by a three-phase analysis motivated by \citet{stoger2021small} (\Cref{thm-fit-ground-truth}).
%In the second stage, we characterize how GD behaves after the top-$s$ components have been discovered. % (\Cref{main-lemma}). 
%The main technical results for this phase is stated in \Cref{main-lemma}.
%Let $\mX_s = \left[ \vv_1, \vv_2,\cdots, \vv_s\right]$ be the top-$s$ components of the ground, and we use
%$\bm{\Sigma}_s = \diag{\sigma_1,\sigma_2,\cdots,\sigma_s}$ to denote the diagonal matrix consisting of
%the singular values of $\mX_s$ and
%use $\bm{\Sigma}_{s,\perp}=\diag{\sigma_{s+1},\sigma_{s+2},\cdots,\sigma_{r_{*}}}$
%to denote the diagonal matrix consisting of the singular values of $\mX$ that do not appear in $\mX_s$.
\begin{comment}
    It is not surprising that the bound in \Cref{thm-fit-ground-truth} is not $o(1)$ when $\alpha\to 0$, because in general $\mZ_s \neq \mX_s \mX_s^{\top}$ due to measurement error. As a result, according to \Cref{main-informal}, when $\alpha\to 0$, we should expect that GD visits an $o(1)$ neighborhood of $\mZ_s$ rather than $\mX_s\mX_s^{\top}$. Indeed, with a measurement error of $\delta$, intuitively we have that $\left\|\mZ_s-\mX_s\mX_s^{\top}\right\|_F \lesssim \delta$, which is consistent with the bound of \Cref{thm-fit-ground-truth}.
\end{comment}
%in a simpler case: the model 
%of 
%$\mU_t\mU_t^\top$ to $\mZ_{\hr}^*$
%consider the simpler setting where the model
%is \textit{under-parameterized}, \emph{i.e.,} $\hr\leq r^*$ and show that
%$\mU_t\mU_t^\top$ would eventually converge to $\mZ_{\hr}^*$.
%\zhiyuan{check proof sketch environment and unify its usage }
We first prove \Cref{main-thm-cor} which can be directly derived by combining
the lemmas in \Cref{subsec:key-lemma}.


\begin{proof}[Proof Sketch of \Cref{main-thm-cor}]
    For any global minimizer $\mU_{\hr}^*$ of \Cref{matrix-sensing}, we have
    \begin{align*}
        &~~~~~\mathrm{dist}(\mU_{\hr}^*,\mU_{\alpha,\hat{T}_{\alpha}^{\hr}}) \\
        &\le (2\sqrt{2}-2)^{-1/2} \sigma_{\min}^{-1}\left(\mU_{\hr}^*\right)
        \left\| \mU_{\alpha,\hat{T}_{\alpha}^{\hr}}\mU_{\alpha,\hat{T}_{\alpha}^{\hr}}^\top - \mZ_{\hr}^*\right\|_F \\
        &\le \O(\kappa^{\frac{1}{2}}\|\mX\|^{-1}) \cdot \O(\kappa^3 r_*\delta\|\mX\|^2) \\
        &= \O(\kappa^{3.5} r_*\delta\|\mX\|),
    \end{align*}
    where the first inequality is due to \Cref{procrutes-property} 
    and the second one is due to 
    \Cref{cor:minima-close} and \Cref{main-lemma}.

    %(see \Cref{approx-rank-s-cor}). %\zhiyuan{this deduction doesn't sound correct, $\mU_{\alpha,\hat{T}_{\alpha}^{\hr}}$ can be different up to a rotation for different $\alpha$.}
    \Cref{asmp:rip} and \Cref{landscape-main-thm} then imply that $\mU_{\alpha,\hat{T}_{\alpha}^{\hr}}$ lies in the small neighborhood of the set of global minimizers of $f=f_{\hr}$, in which the RSI holds.
    %Moreover, we can show that within a neighborhood of $\mU_{\alpha,\hr}^*$ with \textit{constant} radius, $f$ satisfies a Polyak-\L{}ojasiewicz (PL) type condition (taking $s=\hr$ in \Cref{landscape-main-thm}), and the global minimizer of $f$ is unique up to orthogonal transformation.
    %On the other hand, by taking $s=\hr$ in
    %\Cref{landscape-main-thm}, we can see that within a neighborhood of $\mU_{\alpha,\hr}^*$ with \textit{constant} radius, $f$ satisfies a Polyak-\L{}ojasiewicz (PL) type condition with respect to the procrutes distance defined in \Cref{def-procrutes}, and the global minimizer of $f$ is unique up to orthogonal transformation. 
    Following a standard non-convex optimization analysis~\citep{karimi2016linear},
    we can show that GD converges linearly to $\argmin f_{\hr}$ (in the Procrustes distance), which yields the
    conclusion.
    %\zhiyuan{PL condition doesn't imply it will converge to the $U^*_{\hat r}$. You need to mention all minimizers essentially have the same form.}
\end{proof}

Now we turn to prove \Cref{main_result}.
While $f$ is not necessarily local RSI,  we use a low-rank approximation for $\mU_{t}$ and associate the dynamics in this neighborhood with the GD dynamics of $f_s$.
 %\zhiyuan{don't say always, it doesn't sound correct, maybe GD follows low-rank traj until XXX time point}
%Moreover, $\hat{\mU}^*_s \hat{\mU}^{* \top}_s$ always equals the best rank-$s$ solution $\mZ_s^*$.



%\kaifeng{mention landscape result}



\begin{proof}[Proof sketch of \Cref{main_result}]
    Recall that by \Cref{main-lemma}, $\mU_{\alpha,\hat{T}_{\alpha}^s}$ is
    approximately rank-$s$. So there must exist a matrix $\bar{\mU}_{\alpha,0} \in
    \R^{d\times \hr}$ with $\rank{\bar{\mU}_{\alpha,0}} \leq s$ such that
    \begin{equation}
        \label{eq:proof-main-result-1}
        \bar{\mU}_{\alpha,0}\bar{\mU}_{\alpha,0}^\top - \mU_{\alpha,T_{\alpha}^s}\mU_{\alpha,T_{\alpha}^s}^\top = o(1) \quad \text{as }\alpha\to 0.
    \end{equation}
    Indeed, we can let $\bar{\mU}_{\alpha,t}$
    be the parallel component of $\mU_{\alpha,T_{\alpha}^s}$
    because
    the orthogonal component stays $o(1)$ (see the discussions following
    \Cref{ut-decompose} and \Cref{main:refinement-main-cor} for details).
    
    %\mU_{\alpha,t+\hat{T}_{\alpha}^s}\mW_{\alpha,t+\hat{T}_{\alpha}^s}\mW_{\alpha,t+\hat{T}_{\alpha}^s}^\top\in\R^{d\times
    %\hr}$ for all $0 \geq t \geq -\hat{T}_{\alpha}^s$, where $\mW_{\alpha,t} =
    %\mW_{\mV_{\mX_s}^{\top}\mU_{\alpha,t}}$ as defined in \Cref{ut-decompose}.

    Let $\left\{\bar{\mU}_{\alpha,t}\right\}_{t\geq 0}$ be the trajectory of GD
    with step size $\mu$, initialized at $\bar{\mU}_{\alpha,0}$.
    Since the gradient of the objective function $f$ is locally  Lipschitz,
    the solution obtained by the two GD trajectories
    $\{\bar{\mU}_{\alpha,t}\}_{t\geq 0}$ and
    $\{\mU_{\alpha,\hat{T}_{\alpha}^s+t}\}_{t\geq 0}$ will remain $o(1)$-close for at least constantly many steps. Indeed we can show that they will keep $o(1)$ close for some $\bar{t}_{\alpha} = \omega(1)$ steps, \emph{i.e.}, 
    for all $t \in [0, \bar{t}_{\alpha}]$,
    \begin{equation}
        \label{main-lemma-approx}
        \bar{\mU}_{\alpha,t}\bar{\mU}_{\alpha,t}^{\top}- \mU_{\alpha,\hat{T}_{\alpha}^s+t}\mU_{\alpha,\hat{T}_{\alpha}^s+t}^{\top} = o(1).
    \end{equation}
    %until $t = \Theta\left(\log\frac{1}{\alpha}\right)$. %\zhiyuan{describe the time threshold, like $\log 1/\alpha$}
    From \Cref{GD} it is evident that GD initialized at $\bar{\mU}_{\alpha,0}$
    actually lives in the space of matrices with rank $\le s$. Indeed we can
  identify its dynamics with another GD on $f_s$ (defined in
    \Cref{under-param-sensing}). Concretely, let $\hat{\mU}_{\alpha,0}
    \in \R^{d\times s}$ be a matrix so that $\hat{\mU}_{\alpha,0}\hat{\mU}_{\alpha,0}^\top
    = \bar{\mU}_{\alpha,0}\bar{\mU}_{\alpha,0}^\top$, and let
    $\{\hat{\mU}_{\alpha,t}\}_{t\geq 0}$ be the trajectory of GD that optimizes $f_s$ with step size $\mu$ starting from $\hat{\mU}_{\alpha,0}$.
    Then we have
    $\hat{\mU}_{\alpha,t}\hat{\mU}_{\alpha,t}^\top =
    \bar{\mU}_{\alpha,t}\bar{\mU}_{\alpha,t}^\top$ for all $t\geq 0$.

    We can now apply our landscape results for $f_s$ to analyze
    the GD trajectory $\{\hat{\mU}_{\alpha,t}\}_{t\geq 0}$. By
    \Cref{eq:proof-main-result-1} and \Cref{main-lemma}, we have
    $\left\|\hat{\mU}_{\alpha,0}\hat{\mU}_{\alpha,0}^{\top} - \mZ_s^*\right\|_F
    = \O(\kappa^3 r_*\delta\|\mX\|^2)$, so using a similar argument as in the
    proof sketch of \Cref{main-thm-cor},
    \Cref{cor:minima-close,procrutes-property} imply that the initialization
    $\hat{\mU}_{\alpha,0}$ is within an $\O\left(\kappa^{3.5}
    r_*\delta\|\mX\|^2\right)$ neighborhood of the set of global minimizers of
    $f_s(\mU)$. From \Cref{asmp:rip,landscape-main-thm} we know that that
    $f_s(\mU)$ satisfies a local RSI condition in this neighborhood, so
    following standard non-convex optimization analysis
    \citep{karimi2016linear}, we can show that
    $\{\hat{\mU}_{\alpha,t}\}_{t\geq 0}$ converges linearly to its
    set of global minimizers in the Procrustes distance. We need to choose a
    time $t$ such that \Cref{main-lemma-approx} remains true while this linear
    convergence process takes place for sufficiently many steps. This is possible since
    $\bar{t}_{\alpha} = \omega(1)$; indeed we can show that there always exists
    some $t=t_{\alpha}^s \leq \bar{t}_{\alpha}$ such that both
    $\left\|\hat{\mU}_{\alpha,t}\hat{\mU}_{\alpha,t}^{\top}-
    \mU_{\alpha,\hat{T}_{\alpha}^s+t}\mU_{\alpha,\hat{T}_{\alpha}^s+t}^{\top}\right\|_F$
    and $\left\|\hat{\mU}_{\alpha,t}-\bm{U}_s^*\right\|_F$ are bounded by
    $\O(\alpha^{\frac{1}{M\kappa^2}})$. Hence
    $\left\|\mU_{\alpha,t}\mU_{\alpha,t}^\top-\mZ_s^*\right\|_F = \O(\alpha^{\frac{1}{M\kappa^2}})$ when
    $t=T_{\alpha}^s:=\hat{T}_{\alpha}^s+t_{\alpha}^s$. 
    
    %\zhiyuan{only for $s$ smaller than $\hat r\wedge r^*$}
    For $1\leq s < \hr\wedge r_*$ and $t\leq t_{\alpha}^s$, since
    \Cref{main-lemma-approx} holds and $\rank{\hat{\mU}_{\alpha,t}}\leq s$, we
    have $\max_{1\leq t\leq
    T_{\alpha}^s}\sigma_{s+1}\left(\mU_{\alpha,t}\right) \to 0$ as $\alpha\to 0$.
    Finally, by \Cref{lemma:minima-close,asmp:rip} we have
    $\left\|\mZ_{s+1}^*-\mX_{s+1}\mX_{s+1}^\top\right\|
    = \O(\delta\kappa\sqrt{r_*})
    = \O(\kappa^{-1}\|\mX\|^2)$, so $\sigma_{s+1}(\mZ_{s+1}^*)\gtrsim \sigma_{s+1}^2$. Therefore, $\mU_{\alpha,t}\mU_{\alpha,t}^\top$ cannot be
    close to $\mZ_{s+1}^*$ when $t \leq T_{\alpha}^s$, so we must have
    $T_{\alpha}^{s+1}>T_{\alpha}^s$. This completes the proof of
    \Cref{main_result}. 
\end{proof}
%Equipped with \Cref{thm-fit-ground-truth,main-lemma}, we can now prove \Cref{main_result}. \zhiyuan{Why is this discussion not a part of the proof sketch? Probably the entire section 4 is just theorem 4.1 and its proof sketch?}



%By \Cref{main-lemma} we note for $t \leq T_{\alpha}^s$, $\mU_{\alpha,t}$ is always approximately rank-$s$ \emph{i.e.} $\sigma_{s+1}(\mU_{\alpha,t})=o(1)$, where $\sigma_i(\mA)$ denotes the $i$-th largest singular value of a matrix $\mA$. On the other hand, $\mZ_{s+1}^*$ (defined in \Cref{def:best-rank}) satisfies %This is because we can decompose $\mU_t$ into a parallel component and an orthogonal component (cf. proof sketch of \Cref{thm-fit-ground-truth}); \zhiyuan{ideally we should only use the lemma but not the analysis in the lemma to prove the main theorem. Otherwise the lemma doesn't seem to be useful, or the part we are using should be added into the statement of the lemma} the former has rank $\leq s$ while the latter remains $o(1)$. 
%\zhiyuan{in general too much notation, consider giving them names and  mention the name together with the symbols in the main text}
%\zhiyuan{not sure if the proof is aligned with the theorem statement correctly. Thm 4.1 only say such $T^s_\alpha$ exists, but doesn't claim that it cannot be go to the solution of rank $s+1$ before going to the solution of rank $s$?}
%\zhiyuan{lemma 4.2 not used in the proof sketch}

%\zhiyuan{explain how do we get this proposition. Is this an obvious the proposition? what is the connection between the proposition and main theorem?}

==> Sections/main-result.tex <==
In this section, we present our main theorem, following the theoretical setup in \Cref{sec-prelim}.

\begin{theorem} \label{main_result}
Under \Cref{asmp:rip,asmp-full-rank},
consider GD~\Cref{GD}
with learning rate $\mu\leq \frac{1}{10^{3}  \normsm{\mZ^*}}$ and initialization $\mU_{\alpha, 0} = \alpha \bmU$
for solving the matrix sensing problem~\Cref{matrix-sensing}.
There exists a universal constant $c>0$, a constant $C$ (depending on $\hr$ and $\kappa$) %, an exponent $\gamma \ge \frac{1}{10 \kappa}$ 
and a sequence of time points $T_{\alpha}^1<T_{\alpha}^2<\cdots<T_{\alpha}^{\hr\wedge r_*}$ %(depending on $\alpha$)
such that
for all $1 \le s \le \hr \land r_*$, 
the following holds when $\alpha \lesssim \rho^{-c\kappa}$:
\begin{equation}
    \normF{\mU_{\alpha, T_{\alpha}^{s}} \mU_{\alpha, T_{\alpha}^{s}}^\top - \mZ_s^*} \le C \alpha^\frac{1}{10\kappa}.
\end{equation}


%with initialization $\mU_{\alpha, t} = \alpha \mU$,
%there exist positive integers $T_{\alpha}^1<T_{\alpha}^2<\cdots<T_{\alpha}^{r\wedge r_*}$ such that $\lim_{\alpha\to 0}\max_{1\leq i\leq r\wedge r_*}\left\|\mU_{\alpha,T_{\alpha}^i}\mU_{\alpha,T_{\alpha}^i}^\top-\mZ_i\right\| = 0$
\end{theorem}
%\zhiyuan{@jikai, (1) no need to introduce $\gamma$ here, just use $\alpha^{\frac{1}{10\kappa}}$; (2) $T_\alpha$ depending on $\alpha$ seems trivial; (3). what is $r$; (4) $c$ undefined}
Compared with existing works \citep{li2018algorithmic,stoger2021small}, our
result characterizes the complete learning dynamics of GD and reveals an
incremental learning mechanism, \emph{i.e.}, GD starts from learning simple
solutions and then gradually increasing the complexity of search space until it
finds the ground truth. 

%From an optimization perspective, our analysis shows that GD follows a saddle-to-saddle dynamics \citep{jacot2021deep}. Theoretical studies of this dynamics are often restricted to the rank-$1$ case, since extending to higher ranks requires knowledge on how GD approaches the rank-$1$ saddle \citep{li2020towards}. We show that for matrix sensing problems, GD approaches the rank-$s$ saddle through a specific trajectory that approximately lies in the rank-$s$ solution space, which in turn allows GD to efficiently escaping it. The proof idea of \Cref{thm-main} is similar to ~\cite[Theorem 5.6]{li2020towards} which shows that GF with infinitesimal initialization behaves like a rank-$1$ GF, but it is unknown whether the rank-$1$ GF converges to the minimizer for general PSD-constrained optimization problems.

\begin{comment}
\begin{remark}[Finite-time guarantee for recovering the ground-truth]
    
    Define the `hitting time' $T_{\alpha}^* = \inf\left\{ t\geq 0: \left\| \mU_{\alpha,t} \mU_{\alpha,t}^{\top} - \mZ \right\|_F \leq C\alpha^{\gamma_s}\right\}$ for rank $s$. From our proofs in the Appendix, we can derive an estimate of $T_{\alpha}^*$. Firstly, the \textit{spectral phase} ends at $T_0 = \Theta\left( \frac{1}{\mu\|\mX\|^2}\log\frac{1}{\alpha\rho}\right)$ by \Cref{spectral-end}. Second, by \Cref{signal-main}, the lasting time of the \textit{parallel improvement phase} is $\O\left(\frac{1}{\mu\sigma_s^2}\log\alpha^{-1}\right)$. The refinement phase lasts for $\O\left( \frac{1}{\mu\tau_s}\log\left(r_*\kappa_s\right)\right)$ as shown in the proof of \Cref{main-thm-formal}. Finally, convergence to $o(1)$ ($\alpha\to 0$) neighborhood of rank-$s$ global minimizer of $f_s$ is approximately low-rank and locally PL, thus it takes time $\O\left(\frac{1}{\mu\kappa_s\|\mX\|^2}\log\frac{1}{\alpha}\right)$ (cf. \Cref{appsec-main-proof}). Combining all the bounds above, we can deduce that $T_{\alpha}^* \lesssim \frac{1}{\mu\sigma_s^2}\log\frac{1}{\alpha}$ for small $\alpha$.
\end{remark}
\end{comment}



Now we outline the proof of our main theorem. In the following, we fix an
integer $1\leq s \leq \hr\wedge r_*$ and show the existence of $T_{\alpha}^s > 0$
such that $\lim_{\alpha\to
0} \normF{\mU_{\alpha,T_{\alpha}^s}\mU_{\alpha,T_{\alpha}^s}^\top-\mZ^*_s} =
0$. We then show that $T_{\alpha}^s$ is monotone increasing in $s$ for any fixed
$\alpha$.

Our analysis for the rank-$s$ case divides the training dynamics into two stages.
In the first stage, GD starts from small
initialization and recovers the top-$s$ components of $\mZ^*$ with
$\O(\kappa^2\sqrt{r_*}\delta)$ error. 
%We prove this result by a three-phase analysis motivated by \citet{stoger2021small} (\Cref{thm-fit-ground-truth}).
In the second stage, we characterize how GD behaves after the top-$s$ components
have been discovered. % (\Cref{main-lemma}). 
%The main technical results for this phase is stated in \Cref{main-lemma}.
%Let $\mX_s = \left[ \vv_1, \vv_2,\cdots, \vv_s\right]$ be the top-$s$ components of the ground, and we use
%$\bm{\Sigma}_s = \diag{\sigma_1,\sigma_2,\cdots,\sigma_s}$ to denote the diagonal matrix consisting of
%the singular values of $\mX_s$ and
%use $\bm{\Sigma}_{s,\perp}=\diag{\sigma_{s+1},\sigma_{s+2},\cdots,\sigma_{r_{*}}}$
%to denote the diagonal matrix consisting of the singular values of $\mX$ that do not appear in $\mX_s$.

\subsection{First Stage}
The following lemma states the result for the first stage.
%Our first lemma states that
%With small initialization, GD is able to fit the top-$s$ components of the ground truth with an error bound that scales linearly in $\delta$. 
%\kaifeng{I removed the definition of $\tau$, $\mSigma_s$, $\mSigma_{s,\perp}$ here. Define it when you use it.}
\begin{lemma}
\label{thm-fit-ground-truth}
Under \Cref{asmp:rip,asmp-full-rank}, 
if the initialization scale $\alpha$ is sufficiently small,
then for all $1\leq s\leq \hr\wedge r_*$ there exists a time $T_{\alpha}^s \in\mathbb{Z}_{+}$ such that
\begin{equation}
    \notag
    \left\|\mX_{s} \mX_{s}^{\top} - \mU_{T_{\alpha}^s} \mU_{T_{\alpha}^s}^{\top}\right\|_F \leq \kappa^{2}\sqrt{r_*}\|\mX\|^2\delta.
\end{equation}
\end{lemma}

\begin{proof-sketch}
The proof roughly follows the three-phase analysis in \citet{stoger2021small},
with some technical modifications. Starting from a small initialization, GD
initially behaves similar to power iteration since $\mU_{t+1} = (\mI + \mu \mM_t) \mU_t \approx
(\mI+\mu\mM)\mU_t$,
where $\mM := \A^*\A(\mX\mX^{\top})$ is a symmetric matrix.
Let $\mM=\sum_{k=1}^d \hat{\sigma}_k^2
\hat{\vv}_k\hat{\vv}_k^{\top}$ be the eigendecomposition of $\mM$. Then we have
\begin{equation}
    \label{main-spectral-eq}
    \mU_T \approx (\mI+\mu\mM)^{T}\mU_0 = \sum_{i=1}^d (1+\mu\hat{\sigma}_i^2)^{T} \hat{\vv}_i\hat{\vv}_i^{\top}\mU_0 \approx \sum_{i=1}^s (1+\mu\hat{\sigma}_i^2)^{T} \hat{\vv}_i\hat{\vv}_i^{\top}\mU_0
\end{equation}
where the last step holds because it can be shown that $1 + \mu \hat{\sigma}_s > 1 + \mu \hat{\sigma}_{s+1}$,
causing an exponential separation between the magnitude of the top-$s$ and the remaining components.

When \Cref{main-spectral-eq} no longer holds, we enter 
a new phase which we call the \textit{parallel improvement phase}. 
We consider the decomposition $\mU_t = \mU_t\mW_t\mW_t^{\top}+\mU_t\mW_{t,\perp}\mW_{t,\perp}^{\top}$,
where %$\mW_t \in \R^{r\times s}$ is defined by 
$\mW_t := \mW_{\mV_{\mX_s}^{\top}\mU_t} \in \R^{\hr \times s}$
is the matrix consisting of the right singular vectors of $\mV_{\mX_s}^{\top}\mU_t$ (\Cref{def:svd})
and $\mW_{t,\perp} \in \R^{\hr \times (\hr-s)}$ is an orthogonal complement of $\mW_t$.

%the SVD $\mV_{\mX_s}^{\top}\mU_t=\mV_t\bm{\Sigma}_t\mW_t^{\top}$. 

Assume $\mX_s = \left[ \sigma_1\ve_1, \cdots, \sigma_s \ve_s \right]$ without loss of generality. The columns of $\mW_t$ is an orthogonal basis of the subspace spanned by the first $s$ rows of $\mU_t$. Each vector in $\R^r$ can be decomposed as a parallel component and an orthogonal component w.r.t. this subspace. Intuitively, the row vectors of $\mU_t\mW_t$ are the parallel components of the row vectors in $\mU_t$; we call $\mU_t\mW_t$ the \textit{parallel component}. For similar reasons, $\mU_t\mW_{t,\perp}$ will be referred to as the \textit{orthogonal component}.  More discussions for this decomposition are given in \Cref{appsec-main-idea}. 

By the end of the spectral phase we have $\sigma_{\min}\left(\mU_t\mW_t\right)
\gg \left\|\mU_t\mW_{t,\perp}\right\|$, and moreover, we show in
\Cref{subsec:improve} that the parallel component grows exponentially
faster than the orthogonal component, \emph{i.e.,}
$\frac{\sigma_{\min}\left(\mU_t\mW_t\right)}{\left\|\mU_t\mW_{t,\perp}\right\|}$
is exponential in $t$, until the former reaches a constant scale. 

After $\sigma_{\min}\left(\mU_t\mW_t\right)=\Theta(1)$, we enter the
\textit{refinement phase} where we show in \Cref{subsec:refine} that
$\normF{\mX_{s} \mX_{s}^{\top} - \mU_{t} \mU_{t}^{\top}}$ decreases linearly
to $\O\left(\kappa^{2}\sqrt{r_*}\|\mX\|^2\delta\right)$. The conclusion then follows. 
\end{proof-sketch}


\begin{comment}
    It is not surprising that the bound in \Cref{thm-fit-ground-truth} is not $o(1)$ when $\alpha\to 0$, because in general $\mZ_s \neq \mX_s \mX_s^{\top}$ due to measurement error. As a result, according to \Cref{main-informal}, when $\alpha\to 0$, we should expect that GD visits an $o(1)$ neighborhood of $\mZ_s$ rather than $\mX_s\mX_s^{\top}$. Indeed, with a measurement error of $\delta$, intuitively we have that $\left\|\mZ_s-\mX_s\mX_s^{\top}\right\|_F \lesssim \delta$, which is consistent with the bound of \Cref{thm-fit-ground-truth}.
\end{comment}

\subsection{Second Stage}
\Cref{thm-fit-ground-truth} shows the convergence of $\mU_t \mU_t^\top$ to a
neighborhood of $\mX_s\mX_s^\top$ with \textit{constant} radius. In the second
stage, we use a low-rank approximation for $\mU_{\alpha, t}$
and associate the dynamics in this neighborhood
with the GD dynamics of the following under-parameterized matrix sensing
loss:
\begin{equation}
    \label{under-param-sensing}
    f_s(\mU) = \frac{1}{4}\left\|\A(\mZ^*-\mU\mU^{\top})\right\|_2^2,\quad \mU\in\R^{d\times s},
\end{equation}
It can be shown that the global minimizer of $f_s$ is unique up to rotation, i.e.,
if $\hat{\mU}^*_s$ is a global minimizer of $f_s$, then any other global minimizer can be written as
$\hat{\mU}^*_s \mR$ for some orthogonal matrix $\mR \in \R^{s \times s}$.
Moreover, $\hat{\mU}^*_s \hat{\mU}^{* \top}_s$ always equals the best rank-$s$ solution $\mZ_s^*$.


The following lemma states that the GD trajectory until $T_{\alpha}^s$ is approximately low rank. We will use this lemma to show that GD on $f_s$ starting from this low-rank
approximation closely tracks $\mU_{\alpha, t}$ for $t \ge T_{\alpha}$ until convergence to the global minimizer of $f_s$.

\begin{lemma} \label{main-lemma}
There exists $\hat{\mU}_{\alpha,t} \in \R^{d \times s}$
and $\hat{\mR}_{\alpha,t} \in \R^{s \times \hr}$ for each $\alpha > 0$ and $t \in [-T_\alpha^s,0]$ 
%to approximate $\mU_{\alpha, t+T_{\alpha}^s}$ as $\hat{\mU}_{\alpha,t} \hat{\mR}_{\alpha,r}$ in the sense
such that $\lim_{\alpha \to 0} \max_{t\in[-T_\alpha^s,0]} \normF{\hat{\mU}_{\alpha, t}\hat{\mR}_{\alpha,t} - \mU_{\alpha, t+T_{\alpha}^s}} = 0$, where $T_\alpha^s$ is defined in \Cref{thm-fit-ground-truth}.
Moreover, we have 
$\normF{\hat{\mU}_{\alpha,0} - \mU_s^*} \lesssim \kappa^2\sqrt{r_*}\|\mX\|\delta$
for some global minimizer $\mU_s^*$ of $f_s$ and $\hat{\mR}_{\alpha,t}\hat{\mR}_{\alpha,t}^\top = \mI$.%\zhiyuan{$T_\alpha$ not defined}
\end{lemma}

\begin{proof-sketch}
    The approximation is done by setting $\hat{\mU}_{\alpha,t} = \mU_{\alpha,t+T_{\alpha}^s}\mW_{\alpha,t+T_{\alpha}^s}$ and $\hat{\mR}_{\alpha,t} = \mW_{\alpha,t+T_{\alpha}^s}^{\top}$
    because the orthogonal term $\mU_{\alpha,t'}\mW_{\alpha,t',\perp}$ is $o(1)$ for $t'\in[0,T_\alpha^s]$.
    %\textit{(2)} and \textit{(3)} follows from our landscape analysis in \Cref{sec-landscape}.
\end{proof-sketch}

To see why \Cref{main-lemma} is useful, note that it implies that
$\mU_{\alpha,T_{\alpha}^s}$ is approximately rank-$s$, so within a time period
after $T_{\alpha}$, the GD trajectory remains close to another GD initialized at
$\hat{\mU}_{\alpha,0}$ for the rank-$s$ matrix sensing loss
\Cref{under-param-sensing}; that is 
\begin{equation}
    \label{main-lemma-approx}
    \hat{\mU}_{\alpha,t}\hat{\mU}_{\alpha,t}^{\top}\approx \mU_{\alpha,T_{\alpha}^s+t}\mU_{\alpha,T_{\alpha}^s+t}^{\top}
\end{equation}
when $t$ is below a certain time threshold.

It can be derived from \Cref{thm-fit-ground-truth} that the initialization $\hat{\mU}_{\alpha,0}$ is within a
small neighborhood of the global minima of $f_s(\mU)$. Furthermore, \Cref{landscape-main-thm} implies
that $f_s(\mU)$ satisfies a local PL condition, so that GD with good initialization would converge
linearly to its global minima \citep{karimi2016linear}. We need to choose a time
$t$ such that \Cref{main-lemma-approx} remains true while this linear
convergence takes place for sufficiently many steps. We can show that there always exists some $t$ such that both
$\left\|\hat{\mU}_{\alpha,t}\hat{\mU}_{\alpha,t}^{\top}-
\mU_{\alpha,T_{\alpha}^s+t}\mU_{\alpha,T_{\alpha}^s+t}^{\top}\right\|_F$ and
$\left\|\hat{\mU}_{\alpha,t}-\bm{U}_s^*\right\|_F$ are $\O\left(\alpha^{\frac{1}{10\kappa}}\right)$. Equipped with \Cref{thm-fit-ground-truth,main-lemma}, we can now prove \Cref{main_result}. \zhiyuan{Why is this discussion not a part of the proof sketch? Probably the entire section 4 is just theorem 4.1 and its proof sketch?}

%\kaifeng{mention landscape result}



\textbf{\textit{Proof sketch of \Cref{main_result}:}} 
From the above discussion, we can see that there exists a time $t_{\alpha}^s>0$, such that $\left\|\mU_{\alpha,t_\alpha^s}\mU_{\alpha,t_\alpha^s}^{\top}-\mZ_s^*\right\|_F=\O\left(\alpha^{\frac{1}{10\kappa}}\right)$.
Define $T_{\alpha}^s = \inf\left\{ t\geq 0: \left\| \mU_{\alpha,t} \mU_{\alpha,t}^{\top} - \mZ_s^* \right\|_F \leq C\alpha^{\frac{1}{10\kappa}}\right\}$ for rank $1\leq s\leq r\wedge r_*$. It remains to show that when $\alpha$ is small, $T_{\alpha}^s$ is an increasing function in $s$.

Let $\mathcal{M}_s$ be the set of all matrices in $\R^{d\times \hr}$ with rank $\leq s$. First, by \Cref{main-lemma} we note for $t \leq T_{\alpha}^s$, the distance between $\mU_{\alpha,t}$ and $\mathcal{M}_s$ is always $o(1)$ ($\alpha\to 0$). %This is because we can decompose $\mU_t$ into a parallel component and an orthogonal component (cf. proof sketch of \Cref{thm-fit-ground-truth}); \zhiyuan{ideally we should only use the lemma but not the analysis in the lemma to prove the main theorem. Otherwise the lemma doesn't seem to be useful, or the part we are using should be added into the statement of the lemma} the former has rank $\leq s$ while the latter remains $o(1)$. 
On the other hand, $\left\|\mZ_{s+1}^*-\mX_{s+1}\mX_{s+1}^\top\right\|=\O(\delta)$ (cf. \Cref{minima-close}), so $\mZ_{s+1}^*$ is not approximately rank-$s$. Thus $\mU_t\mU_t^\top$ cannot be close to $\mZ_{s+1}^*$ when $t \leq T_{\alpha}^s$. \zhiyuan{what is the definition of $Z_{s+1}^*$? don't understand the last sentence} \zhiyuan{in general too much notation, consider giving them names and  mention the name together with the symbols in the main text}
\\
\zhiyuan{not sure if the proof is aligned with the theorem statement correctly. Thm 4.1 only say such $T^s_\alpha$ exists, but doesn't claim that it cannot be go to the solution of rank $s+1$ before going to the solution of rank $s$?}
%\zhiyuan{lemma 4.2 not used in the proof sketch}
We conclude this section with the following proposition, which states that in the under-parameterized setting, GD converges to the global minimizer of the matrix sensing loss.
\begin{proposition}
\label{main-thm-cor}
    Suppose that $\hr\leq r^*$, then there exists a constant $c=c(\hr,\kappa)>0$ such that when $\alpha<c$, we have $\lim_{t\to +\infty}\mU_{\alpha,t}\mU_{\alpha,t}^{\top}=\mZ_{\hr}^*$.
\end{proposition}
\zhiyuan{explain how do we get this proposition. Is this an obvious the proposition? what is the connection between the proposition and main theorem?}



\kaifeng{old text is in the comment}

\begin{comment}
Now we
show that $\mU_t \mU_t^\top$ converges to $\mZ^*_s$
after that.

\begin{lemma}
\label{main-lemma}
The following statements hold:
\begin{enumerate}[(1).]
\item There exists a rank-$s$ matrix $\widetilde{\mU}_{\alpha} \in \R^{d \times \hr}$ for every $\alpha > 0$ such that $\lim_{\alpha\to 0}\left\|\widetilde{\mU}_{\alpha} - \mU_{\alpha,T_{\alpha}}\right\|_F = 0$, where $T_{\alpha}$ is defined in \Cref{thm-fit-ground-truth}.
\item Let $\hat{\mU}_{\alpha,0}\in\R^{d\times s}$ be such that $\hat{\mU}_{\alpha,0}\hat{\mU}_{\alpha,0}^{\top} = \widetilde{\mU}_{\alpha}\widetilde{\mU}_{\alpha}^{\top}$. Consider under-parameterized matrix sensing loss
then the global minimizer of $f_s$ is unique up to rotation. In other words, for any two global minimizers $\mU_1$ and $\mU_2$, there exists an orthogonal matrix $\mR\in\R^{s\times s}$ such that $\mU_1=\mU_2\mR$. Moreover, there exists a global minimizer $\mU_s^*$ such that $\left\|\hat{\mU}_{\alpha,0} - \mU_s^*\right\|_F \lesssim \kappa^2\sqrt{r_*}\|X\|\delta$.
\item The function $f_s$ satisfies a local Polyak-Lojasiewicz (PL) condition. Specifically, let $\mU\in\R^{d\times s}$ and $\mU_s^*$ be the global minimizer with minimal distance (under $\|\cdot\|_F$) to $\mU$, then we have $\left\langle \nabla f_s(\mU), \mU - \mU_s^*\right\rangle \geq 0.1\tau \left\|\mU-\mU_s^*\right\|_F^2$
whenever $\left\|\mU-\mU_s^*\right\| \leq 10^{-2}\kappa^{-1}\|\mX\|$.
\end{enumerate}
\end{lemma}

\begin{proof-sketch}
    The statement of \textit{(1)} follows directly by choosing $\widetilde{\mU}_0 = \mU_{\alpha,T_{\alpha}}\mW_{\alpha,T_{\alpha}}\mW_{\alpha,T_{\alpha}}^{\top}$ and the observation that the parallel term $\mU_{\alpha,t}\mW_{\alpha,t,\perp}$ is $o(1)$ for $t=T_{\alpha}$. \textit{(2)} and \textit{(3)} follows from our landscape analysis in \Cref{sec-landscape}.
\end{proof-sketch}



%Hence, we arrive at the following theorem

\begin{comment}
\begin{lemma}
    \label{thm-main}
    Under \Cref{asmp:rip,asmp-full-rank}, suppose that $\delta \leq 10^{-7}r_*^{-1}\kappa^{-3}$ and $\mu\leq 10^{-3}\|X\|^{-2}$, then there exists 
    a constant $C = C(r,\kappa)$ such that 
    $\min_{t\geq 0}\left\| \mU_{\alpha,t} \mU_{\alpha,t}^{\top} - \mZ_s \right\|_F \leq C\alpha^{\gamma}$
    for all sufficiently small $\alpha \lesssim \rho^{-c\kappa}$, where $\gamma\geq 0.1\kappa^{-1}$.
\end{lemma}

Equipped with \Cref{thm-fit-ground-truth,main-lemma}, we can now prove \Cref{main_result}.

\textbf{\textit{Proof sketch of \Cref{main_result}:}} Define $T_{\alpha}^s = \inf\left\{ t\geq 0: \left\| \mU_{\alpha,t} \mU_{\alpha,t}^{\top} - \mZ \right\|_F \leq C\alpha^{\gamma_s}\right\}$ for rank $1\leq s\leq r\wedge r_*$. It remains to show that when $\alpha$ is small, $T_{\alpha}^s$ is an increasing function in $s$.

Let $\mathcal{M}_s$ be the set of all matrices in $\R^{d\times r}$ with rank $\leq s$. First, we note for $t \leq T_{\alpha}^s$, the distance between $\mU_t$ and $\mathcal{M}_s$ is always $o(1)$ ($\alpha\to 0$). This is because we can decompose $\mU_t$ into a parallel component and an orthogonal component (cf. proof sketch of \Cref{thm-fit-ground-truth}); the former has rank $\leq s$ while the latter remains $o(1)$. On the other hand, $\left\|\mZ_{s+1}-\mX_{s+1}\mX_{s+1}^\top\right\|=\O(\delta)$ (cf. \Cref{minima-close}), so $\mZ_{s+1}$ is not approximately rank-$s$. Thus $\mU_t\mU_t^\top$ cannot find $\mZ_{s+1}$ when $t \leq T_{\alpha}^s$.
\\

%Contrary to what classical statistical learning theory suggests, it is empirically observed that highly expressive and over-parameterized models such as deep neural networks are still able to achieve good generalization performance. It is suggested that this is probably due to the implicit regularization of optimization algorithms. 

\end{comment}


==> Sections/proof_sketch_main.tex <==
In this section, we outline the proof sketch of \Cref{main-lemma}. We divide the
GD dynamics intro three phases and characterize the dynamics separately.
Proof details for these three phases can be found in
\Cref{subsec:spectral,subsec:improve,subsec:refine}.
%the SVD $\mV_{\mX_s}^{\top}\mU_t=\mV_t\bm{\Sigma}_t\mW_t^{\top}$. 
%Assume $\mX_s = \left[ \sigma_1\ve_1, \cdots, \sigma_s \ve_s \right]$ without loss of generality, then the columns of $\mW_t$ is an orthogonal basis of the subspace spanned by the first $s$ rows of $\mU_t$. Each vector in $\R^r$ can be decomposed as a parallel component and an orthogonal component w.r.t. this subspace. Intuitively, the row vectors of $\mU_t\mW_t$ are the parallel components of the row vectors in $\mU_t$; we call $\mU_t\mW_t$ the \textit{parallel component}. For similar reasons, $\mU_t\mW_{t,\perp}$ will be referred to as the \textit{orthogonal component}. In the following, we investigate the dynamics of GD in three phases.

\subsection{The spectral phase}

Starting from a small initialization, GD
initially behaves similarly to power iteration since $\mU_{t+1} = (\mI + \mu \mM_t) \mU_t \approx
(\mI+\mu\mM)\mU_t$,
where $\mM := \A^*\A(\mX\mX^{\top})$ is a symmetric matrix.
Let $\mM=\sum_{k=1}^d \hat{\sigma}_k^2
\hat{\vv}_k\hat{\vv}_k^{\top}$ be the eigendecomposition of $\mM$, where $\hat{\sigma}_1\geq \hat{\sigma}_2 \geq \cdots\geq\hat{\sigma}_d\geq 0$. Using our assumption on $\delta$ (\Cref{asmp:rip}), we can show that $\left|\sigma_i-\hat{\sigma}_i\right|, 1\leq i\leq s$ are sufficiently small so that $\hat{\sigma}_i$'s are positive and well-separated. Then we have
\begin{equation}
    \label{main-spectral-eq}
    \begin{aligned}
        \mU_T \approx (\mI+\mu\mM)^{T}\mU_0
        &= \sum_{i=1}^d (1+\mu\hat{\sigma}_i^2)^{T} \hat{\vv}_i\hat{\vv}_i^{\top}\mU_0 \\
        &\approx \sum_{i=1}^s (1+\mu\hat{\sigma}_i^2)^{T} \hat{\vv}_i\hat{\vv}_i^{\top}\mU_0,
    \end{aligned}
\end{equation}
where the last step holds because $(1 + \mu \hat{\sigma}_s)^T \gg (1 + \mu \hat{\sigma}_{s+1})^T$. In other words, we can expect that there is an exponential separation between the parallel and orthogonal component of $\mU_T$. Formally, we can prove the following property at the end of the spectral phase:

\begin{lemma}[\Cref{spectral-end}, simplified version]
\label{main:spectral-end}
Suppose that \Cref{asmp:rip,asmp-full-rank,asmp:step-size} hold. Then there
exist positive constants $C_i = C_i(\mX,\bar{\mU}), \gamma_i =
\gamma_i(\mX,\bar{\mU}), i=2,3$ independent of $\alpha$ such that
$\gamma_2<\gamma_3$ and the following inequalities hold for $t =
T_{\alpha}^{\sp} = \O\left( \frac{\log\alpha^{-1}}{\log(1+\mu\|\mX\|^2)}
\right)$ when $\alpha$ is sufficiently small:
\begin{subequations}
    \label{main:induction-base}
    \begin{align*}
    \|\mU_t\| \leq \|\mX\|, &\quad \sigma_{\min}\left( \mU_{t}\mW_{t}\right) \geq C_2\cdot \alpha^{\gamma_2}, \\
    \left\|\mU_{t}\mW_{t,\perp}\right\| \leq C_3\cdot\alpha^{\gamma_3},\text{and} &\quad \left\| \mV_{\mX_s,\perp}^{\top} \mV_{\mU_{t}\mW_{t}}\right\| \leq 200\delta.
    \end{align*}
\end{subequations}
\end{lemma}

\subsection{The parallel improvement phase}

For small $\alpha$, we have $\sigma_{\min}\left(\mU_t\mW_t\right)
\gg \left\|\mU_t\mW_{t,\perp}\right\|$ by the end of the spectral phase. When \Cref{main-spectral-eq} no longer holds, we enter 
a new phase which we call the \textit{parallel improvement phase}. In this phase, the ratio
$\frac{\sigma_{\min}\left(\mU_t\mW_t\right)}{\left\|\mU_t\mW_{t,\perp}\right\|}$
grows exponentially in $t$, until the former reaches a constant scale. Formally, let $T_{\alpha,s}^{\tpi}=\min \left\{t \geqslant 0: \sigma_{\min }^2\left(\mV_{\mX_{s}}^{\top} \mU_{\alpha,t+1}\right)>0.3\kappa^{-1}\|\mX\|^2\right\}$,
then we can prove the following lemma via induction.



\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/low_rank_bias0.png}
        \vspace{-0.6cm}
        \caption[]%
        {{\small $\alpha=1$, $1000$ measurements.}}    
        \label{low_rank0}
    \end{subfigure}
    \qquad
    \begin{subfigure}{0.3\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_bias1.png}
        \vspace{-0.6cm}
        \caption[]%
        {{\small $\alpha=0.1$, $1000$ measurements.}}    
        \label{low_rank1}
    \end{subfigure}
    \qquad
    \begin{subfigure}{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_bias2.png}
        \vspace{-0.6cm}
        \caption[]%
        {{\small $\alpha=0.01$, $1000$ measurements.}}    
        \label{low_rank2}
    \end{subfigure}
    \vskip\baselineskip\vspace{-0.15in}
    \begin{subfigure}{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_bias3.png}
        \vspace{-0.6cm}
        \caption[]%
        {{\small $\alpha=0.001$, $1000$ measurements.}}    
        \label{low_rank3}
    \end{subfigure}
    \qquad
    \begin{subfigure}{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_bias4.png}
        \vspace{-0.6cm}
        \caption[]%
        {{\small $\alpha=0.001$, $2000$ measurements.}}    
        \label{low_rank4}
    \end{subfigure}
    \qquad
    \begin{subfigure}{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_bias5.png}
        \vspace{-0.6cm}
        \caption[]%
        {{\small $\alpha=0.001$, $5000$ measurements.}}    
        \label{low_rank5}
    \end{subfigure}
    \vspace{-0.2cm}
    \caption[]%
    {The evolution of relative error against the best solution of different ranks over time.} 
    \label{low_rank}
    \vspace{-0.4cm}
\end{figure*}


\begin{restatable}[]{lemma}{inductionLemma}
\label{main:induction-lemma}
Suppose that \Cref{asmp:rip,asmp-full-rank,asmp:step-size} hold and let $c_3 = 10^{4}\kappa r_{*}^{\frac{1}{2}} \delta$. Then for sufficiently small $\alpha$,  the following inequalities hold when $T_{\alpha}^{\sp} \leq t < T_{\alpha,s}^{\tpi}$:

\vspace{-0.65cm}

\begin{subequations}
\label{main:induction-eq}
\begin{align}
    &\quad \sigma_{\min }\left(\mV_{\mX_{s}}^{\top} \mU_{t+1}\right)
    \geq \sigma_{\min }\left(\mV_{\mX_{s}}^{\top} \mU_{t+1}\mW_{t}\right) \nonumber\\
    &\qquad \geq \left(1+0.5 \mu\left(\sigma_{s}^{2}+\sigma_{s+1}^{2}\right)\right) \sigma_{\min }\left(\mV_{\mX_{s}}^{\top} \mU_t\right), \label{main:induction-1} \\
    & \quad \left\|\mU_{t+1} \mW_{t+1, \perp}\right\| \nonumber\\
    & \qquad \leq \left(1+\mu \left(0.4 \sigma_s^2+0.6 \sigma_{s+1}^{2}\right)\right)\left\|\mU_{t} \mW_{t,\perp}\right\|,  \label{main:induction-2}\\
    & \quad\left\|\mV_{\mX_s,\perp}^{\top} \mV_{\mU_{t+1}\mW_{t+1}}\right\| \leq c_3,\label{main:induction-3} \\
    &\quad \rank{\mV_{\mX_{s}}^{\top} \mU_{t+1}} = \rank{\mV_{\mX_{s}}^{\top} \mU_{t+1}\mW_{t}} = s.\label{main:induction-4}
\end{align}
\end{subequations}
\end{restatable}


\vspace{-0.25cm}


We can immediately deduce from \Cref{main:spectral-end,main:induction-lemma} that the orthogonal term $\|\mU_t\mW_{t,\perp}\|$ remains $o(1)$ by the end of the parallel improvement phase:

\begin{corollary}[\Cref{refinement-start}, simplified version]
\label{main:refinement-start}
Under the conditions of \Cref{main:induction-lemma}, when $\alpha$ is sufficiently small we have $\left\| \mU_{T_{\alpha,s}^{\tpi}} \mW_{T_{\alpha,s}^{\tpi},\perp}\right\| \leq C_5\cdot \alpha^{\frac{1}{4\kappa}}$
for some constant $C_5 = C_5(\mX,\bar{\mU})$.
\end{corollary}


\begin{figure*}[!t]
    %\vspace{-0.25in}
    \centering
    \begin{subfigure}[c]{0.3\textwidth}  
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_exact1.png}
        \caption[]%
        {{\small $\alpha=0.1$, $1000$ measurements.}}    
        \label{low_rank_exact1}
    \end{subfigure}
    \qquad
    %\vskip\baselineskip\vspace{-0.15in}
    \begin{subfigure}[c]{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_exact2.png}
        \caption[]%
        {{\small $\alpha=0.01$, $1000$ measurements.}}    
        \label{low_rank_exact2}
    \end{subfigure}
    \qquad
    \begin{subfigure}[c]{0.3\textwidth}   
        \centering 
        \includegraphics[width=\textwidth]{Figures/low_rank_exact3.png}
        \caption[]%
        {{\small $\alpha=0.001$, $1000$ measurements.}}    
        \label{low_rank_exact3}
    \end{subfigure}
    \vspace{-0.2cm}
    \caption[]%
    {The evolution of the loss and relative error against best solution of different ranks in the exact-parameterized case $\hr=r_*=5$.}
    \label{low_rank_exact}
    \vspace{-0.4cm}
\end{figure*}

\vspace{-0.3cm}

\subsection{The refinement phase}

After $\sigma_{\min}\left(\mU_t\mW_t\right)$ grows to constant scale, we enter the
\textit{refinement phase} for which we show that
$\normF{\mX_{s} \mX_{s}^{\top} - \mU_{t} \mU_{t}^{\top}}$ keeps decreasing
until it is $\O\left(\delta\kappa^{3}r_*\|\mX\|^2\right)$. Formally, let $\tau=\kappa^{-1}\|\mX\|^2$ and $T_{\alpha, s}^{\mathrm{ft}}=T_{\alpha, s}^{\mathrm{pi}}-\frac{\log \left(10^{-2}\|\boldsymbol{X}\|^{-2} \kappa^{-1} c_3^{-1}\right)}{\log \left(1-\frac{1}{2} \mu \tau\right)}> T_{\alpha, s}^{\mathrm{pi}}$ where $c_3$ is defined in \Cref{main:induction-lemma},
then the following lemma holds.

\begin{restatable}[]{lemma}{refineMain}
    \label{main:refinement-main}
    Suppose that $T_{\alpha,s}^{\tpi}\leq t \leq T_{\alpha, s}^{\mathrm{ft}}$ and all the conditions in \Cref{main:induction-lemma} hold, then we have
    \begin{align}
        &\left\| \mV_{\mX_s}^{\top}( \mX\mX^{\top}-\mU_{t+1}\mU_{t+1}^{\top})\right\|_F \nonumber \\
        \leq &\left( 1-\frac{1}{2}\mu\tau\right)\left\| \mV_{\mX_s}^{\top}\left(\mX \mX^{\top}-\mU_{t} \mU_{t}^{\top}\right)\right\|_F \nonumber\\
        &\quad + 20\mu\|\mX\|^4\left( \delta+5c_3\right) + 2000\mu^2\sqrt{r_*}\|\mX\|^6. \nonumber
    \end{align}
    Moreover, it holds that $\left\|\mU_{t+1}\mW_{t+1,\perp}\right\| \leq (1+\sigma_s^2)\|\mU_t\mW_{t,\perp}\|$ and $\left\| \mV_{\mX_s^\perp}\mV_{\mU_t \mW_t}\right\| \leq c_3$.
\end{restatable}



%\vspace{-0.6cm}
Using \Cref{main:refinement-main}, we arrive at the following result:

\begin{corollary}
\label{main:refinement-main-cor}
    For sufficiently small $\alpha$, at $t=T_{\alpha, s}^{\mathrm{ft}}$ we have $\left\|\boldsymbol{V}_{\boldsymbol{X}_s}^{\top}\left(\boldsymbol{X} \boldsymbol{X}^{\top}-\boldsymbol{U}_{t} \boldsymbol{U}_{t}^{\top}\right)\right\|_F \leq 80 \delta\kappa^3 r_*\|\mX\|^2$ and $\|\mU_t\mW_{t,\perp}\|=o(1)$ ($\alpha\to 0$).
\end{corollary}

\textit{\textbf{Concluding the proof of \Cref{main-lemma}.}} At $t=T_{\alpha, s}^{\mathrm{ft}}$, we have
\begin{subequations}
\label{eq:linear-convergence}
    \begin{align}
    &\quad \left\|\mX_{s} \mX_{s}^{\top}-\mU_{t} \mU_{t}^{\top}\right\|_F \nonumber \\& \leq \left\|\left(\mX_{s} \mX_{s}^{\top}-\mU_{t} \mU_{t}^{\top}\right) \mV_{\mX_{s}} \mV_{\mX_{s}}^{\top}\right\|_F +\left\|\mU_{t} \mU_{t}^{\top} \mV_{\mX_{s}^{\perp}} \mV_{\mX_{s}^{\perp}}^{\top}\right\|_F\nonumber \\
    &\leq \left\|\left(\mX_{s} \mX_{s}^{\top}-\mU_{t} \mU_{t}^{\top}\right) \mV_{\mX_{s}} \mV_{\mX_{s}}^{\top}\right\|_F +\left\|\mV_{\mX_{s}^{\perp}}^{\top} \mU_{t} \mU_{t}^{\top} \mV_{\mX_{s}^{\perp}}\right\|_F\nonumber \\
    &\leq \left\| \mV_{\mX_{s}}^{\top}\left(\mX_{s} \mX_{s}^{\top}-\mU_{t} \mU_{t}^{\top}\right)\right\|_F  \nonumber\\
    &\quad + \sqrt{r_*}\left\|\mV_{\mX_{s}^{\perp}}^{\top} \mU_{t} \mW_{t}\right\|^2+\sqrt{d}\left\|\mV_{\mX_{s}^{\perp}}^{\top} \mU_{t} \mW_{t, \perp}\right\|^2\label{eq:linear-convergence-1} \\
    &\leq \left\| \mV_{\mX_{s}}^{\top}\left(\mX_{s} \mX_{s}^{\top}-\mU_{t} \mU_{t}^{\top}\right)\right\|_F\nonumber \\
    &\quad \! +\! 9\sqrt{r_*}\|\mX\|^2 \left\| \mV_{\mX_s^\perp}\mV_{\mU_t \mW_t}\right\|^2\! +\! \sqrt{d}\| \mU_t \mW_{t,\perp}\|^2\!\!\label{eq:linear-convergence-2}\\
    &= \O\left( \delta\kappa^3 r_*\|\mX\|^2 + \|\mX\|^2 c_3^2\sqrt{r_*}\right) + o(1)\label{eq:linear-convergence-3} \\
    &= \O\left( \delta\kappa^3 r_*\|\mX\|^2\right),\label{eq:linear-convergence-4}
    \end{align}
\end{subequations}
where \Cref{eq:linear-convergence-1} uses $\|\mA\|_F \leq \sqrt{\rank{\mA}}\|\mA\|$, \Cref{eq:linear-convergence-2} uses $\|\mU_t\|\leq 3\|\mX\|$, \Cref{eq:linear-convergence-3} follows from \Cref{main:refinement-main,main:refinement-main-cor} and the last step follows from $c_3=10^4\kappa\sqrt{r_*}\delta$ and \Cref{asmp:rip}.
%\zhiyuan{@jikai, I think we need to explain the last four steps. like why introducing $c_3$? @kaifeng, please read these steps and see if you can understand them}

By \Cref{lemma:minima-close}, the best rank-$s$ solution is close to the matrix factorization minimizer \emph{i.e.} $\left\|\mZ_s^*-\mX_s\mX_s^\top\right\|_F = \O\left(\delta\kappa\sqrt{r_*}\|\mX\|^2\right)$. We thus obtain that $\normF{\mZ_s^* - \mU_{t} \mU_{t}^{\top}} = \O\left(\delta\kappa^3 r_*\|\mX\|^2\right)$. Finally, since $\rank{\mU_t\mW_t}\leq s$ (recall the decomposition \Cref{ut-decompose}), we have $\sigma_{s+1}(\mU_t) \leq \left\|\mU_t\mW_{t,\perp}\right\| = o(1)$. The conclusion follows.


